Verifying Functional Correctness Properties At the Level of Java Bytecode

The breakneck evolution of modern programming languages aggravates the development of deductive verification tools, which struggle to timely and fully support all new language features. To address this challenge, we present ByteBack: a verification technique that works on Java bytecode. Compared to high-level languages, intermediate representations such as bytecode offer a much more limited and stable set of features; hence, they may help decouple the verification process from changes in the source-level language. ByteBack offers a library to specify functional correctness properties at the level of the source code, so that the bytecode is only used as an intermediate representation that the end user does not need to work with. Then, ByteBack reconstructs some of the information about types and expressions that is erased during compilation into bytecode but is necessary to correctly perform verification. Our experiments with an implementation of ByteBack demonstrate that it can successfully verify bytecode compiled from different versions of Java, and including several modern language features that even state-of-the-art Java verifiers (such as KeY and OpenJML) do not directly support$\unicode{x2013}$thus revealing how ByteBack's approach can help keep up verification technology with language evolution.

==> examples/Makefile <==
JFLAGS = 
JC = javac
JRE = java

SOURCES = ClassicCounter.java RecentCounter.java

# clear any default targets for these extensions
.SUFFIXES: .java .class

# target for creating .class files from .java sources
# `make foo.class` will compile foo.java
.java.class:
	$(JC) $(JFLAGS) $*.java

default: run

# compile all targets
compile: $(SOURCES:.java=.class)

run: compile
	@echo "\nRunning classic counter:"
	$(JRE) ClassicCounter
	@echo "\nRunning recent counter:"
	$(JRE) RecentCounter

clean:
	rm -f *.class

.PHONY: clean


==> tables/byteback-model.tex <==
\begin{tabular}{l | l}
  Heap Model & 
\begin{listing}[language=boogie]
type Store = [Reference]<a>[Field a]a
\end{listing}
 \\
  
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:

==> tables/expression-operations.tex <==
\begin{tabular}{llll}
  \textsc{Name}               & \textsc{Jimple}                                           & \textsc{Type} & \textsc{Boogie}                                  \\
  \toprule
  Addition                    & \(\Tr(\G{a + b})\)                                       & *             & \B{$\Tr$(a) +\ $\Tr$(b)}                        \\
  Subtraction                 & \(\Tr(\G{a - b})\)                                       & *             & \B{$\Tr$(a) -\ $\Tr$(b)}                        \\
  Multiplication              & \(\Tr(\G{a * b})\)                                       & *             & \B{$\Tr$(a) *\ $\Tr$(b)}                        \\
  Division                    & \(\Tr(\G{a / b})\)                                       & *             & \B{$\Tr$(a) /\ $\Tr$(b)}                        \\
  Integer Division            & \(\Tr(\G{a / b})\)                                       & \G{int}      & \B{$\Tr$(a) div\ $\Tr$(b)}                      \\
  Negation                    & \(\Tr(\G{-a})\)                                          & *             & \B{-$\Tr$(a)}                                   \\
  Boolean Negation            & \(\Tr(\G{-a})\)                                          & \G{boolean}  & \B{!$\Tr$(a)}                                   \\
  Equality                    & \(\Tr(\G{a == b})\)                                      & *             & \B{$\Tr$(a) ==\ $\Tr$(b)}                       \\
  Inequality                  & \(\Tr(\G{a != b})\)                                      & *             & \B{$\Tr$(a) !=\ $\Tr$(b)}                       \\
  Greater                     & \(\Tr(\G{a > b})\)                                       & *             & \B{$\Tr$(a) >\ $\Tr$(b)}                        \\
  Greater or Equal            & \(\Tr(\G{a >= b})\)                                      & *             & \B{$\Tr$(a) >=\ $\Tr$(b)}                       \\
  Less                        & \(\Tr(\G{a < b})\)                                       & *             & \B{$\Tr$(a) <\ $\Tr$(b)}                        \\
  Less or Equal               & \(\Tr(\G{a <= b})\)                                      & *             & \B{$\Tr$(a) <=\ $\Tr$(b)}                       \\
  Boolean XOR                 & \(\Tr(\G{a \^ b})\)                                      & \G{boolean}  & \B{$\Tr$(a) !=\ $\Tr$(b)}                       \\
  Boolean AND                 & \(\Tr(\G{a \& b})\)                                      & \G{boolean}  & \B{$\Tr$(a) \&\&\ $\Tr$(b)}                     \\
  Boolean OR                  & \(\Tr(\G{a \| b})\)                                      & \G{boolean}  & \B{$\Tr$(a) \|\|\ $\Tr$(b)}                     \\
  Length of Array             & \(\Tr(\G{length(a)})\)                                   & *             & \B{lengthof($\Tr$(a))}                        \\
  Compare                     & \(\Tr(\G{a cmp b})\)                                     & *             & \B{cmp($\Tr$(a),\ $\Tr$(b))}                  \\
  Compare (Greater Than Bias) & \(\Tr(\G{a cmpl b})\)                                    & *             & \B{cmp($\Tr$(a),\ $\Tr$(b))}                  \\
  Compare (Less Than Bias)    & \(\Tr(\G{a cmpg b})\)                                    & *             & \B{cmp($\Tr$(a),\ $\Tr$(b))}                  \\
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:

==> tables/feature-data-short.tex <==
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llcccc}
  \toprule
  \multicolumn{1}{c}{} & & \multicolumn{1}{c}{\textsc{Java}}    & \multicolumn{3}{c}{\textsc{support}}
    \\
                                & \multicolumn{1}{c}{\textsc{feature}} & \multicolumn{1}{c}{\textsc{version}}
                                & KeY                                  & Krakatoa & OpenJML
    \\
  \midrule
  G                            & Generic classes
                                & 5
                                & \suppPart                            & \suppNO  & \suppOK 
    \\
  F                            & Enhanced \J{for} loop
                                & 5
                                & \suppOK                              & \suppNO  & \suppOK 
    \\
  A                            & Varargs
                                & 5
                                & \suppOK                              & \suppNO  & \suppNO 
    \\
  T                           & Generic type inference
                                & 7 
                                & \suppNO                              & \suppNO  & \suppNO
    \\
  % String comparison in \J{switch}
  %                             & 7 
  %                             & \suppNO                              & \suppNO  & \suppNO
  % \\
   D                          & Default methods
                                & 8 
                                & \suppOK                              & \suppNO  & \suppOK
    \\
   L                         & Local type inference
                                & 10 
                                & \suppNO                              & \suppNO  & \suppNO
    \\
   S                          & Switch expressions
                                & 12 
                                & \suppNO                              & \suppNO  & \suppNO
    \\
   Y                         & Switch expressions with \J{yield}
                                & 13
                                & \suppNO                              & \suppNO  & \suppNO
    \\
   P                          & Pattern matching with \J{instanceof}
                                & 14 
                                & \suppNO                              & \suppNO  & \suppNO
    \\
    \bottomrule
\end{tabular}
%%% Local Variables:
%%% mode: plain-tex
%%% TeX-master: t
%%% End:


==> tables/invoke-operations-procedural.tex <==

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:

==> tables/invoke-operations-pure.tex <==
\begin{tabular}{llll}
  \textsc{Name}    & \textsc{Jimple}                           & \textsc{Boogie}                                         \\
  \toprule
  Invoke-Static    & \(\Tr(\G{A.f(p$_1$, $\ldots$, p$_n$)})\) & \B{A.f(heap, $\Tr$(p$_1$), $\ldots$, $\Tr$(p$_n$))}    \\
  Invoke-Virtual   & \(\Tr(\G{a.f(p$_1$, $\ldots$, p$_n$)})\) & \B{A.f(heap, a, $\Tr$(p$_1$), $\ldots$, $\Tr$(p$_n$))} \\
  \hline
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:

==> tables/procedural-expression-conversion.tex <==
\begin{tabular} {lll}
  \textsc{Name}        & \textsc{Jimple}                & \textsc{Boogie}                                    \\
  \toprule
  New Expression       & new C                          & new(C)                                            \\
  New Array Expression & newarray (t) [n]               & array(t, $\Tr$(n))                                \\
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:

==> tables/reference-operations.tex <==
\begin{tabular}{llll}
  \textsc{Name}          & \textsc{Jimple}    & \textsc{Type} & \textsc{Boogie}                                        \\
  \toprule
  Local                  & \(\Tr(\G{a})\)    & *             & \B{a}                                                 \\
  Field Reference        & \(\Tr(\G{a.f})\)  & *             & \B{heap.read(heap,\ $\Tr$(a), f)}                     \\
  Static Field Reference & \(\Tr(\G{A.f})\)  & *             & \B{heap.read(heap,\ type.reference(A), f)}            \\
  Array Reference        & \(\Tr(\G{a[i]})\) & \(\alpha\)    & \B{array.read(heap, a,\ $\Tr$(i))} :\ $\Tr$($\alpha$) \\
  \hline
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:

==> tables/statements-conversion.tex <==
\begin{tabular} {lll}
  \textsc{Name}           & \textsc{Jimple}                & \textsc{Boogie}                                                 \\
  \toprule
  Assignment              & \G{a = b;}                    & \B{a :=\ $\Tr$(b);}                                            \\
  Field Assignment        & \G{a.f = b;}                  & \B{heap = heap.update(heap, a, f,\ $\Tr$(b));}                 \\
  Static Field Assignment & \G{A.f = b;}                  & \B{heap = heap.update(heap, type.reference(A), f,\ $\Tr$(b));} \\
  Array Assignment        & \G{a[i] = b;}                 & \B{heap = array.update(heap, a, i, b);}                        \\
  Return Void Statement   & \G{return;}                   & \B{return;}                                                    \\
  Return Value Statement  & \G{return a;}                 & \B{@ret := a; return;}                                         \\
  Goto Statement          & \G{goto label;}               & \B{goto label;}                                                \\
  If Statement            & \G{if (a) goto label;}        & \B{if (a) \{ goto label; \}}                                   \\
  Invoke Statement        & \G{C.f(p$_1$,$\ldots$,p$_n$)} & \B{call * C.f($\Tr$(p$_1$),$\ldots$,$\Tr$(p$_n$))}              \\
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../byteback"
%%% End:
